FUTURE: Flexible Unlearning for Tree Ensemble

Tree ensembles are widely recognized for their effectiveness in classification tasks, achieving state-of-the-art performance across diverse domains, including bioinformatics, finance, and medical diagnosis. With increasing emphasis on data privacy and the \textit{right to be forgotten}, several unlearning algorithms have been proposed to enable tree ensembles to forget sensitive information. However, existing methods are often tailored to a particular model or rely on the discrete tree structure, making them difficult to generalize to complex ensembles and inefficient for large-scale datasets. To address these limitations, we propose FUTURE, a novel unlearning algorithm for tree ensembles. Specifically, we formulate the problem of forgetting samples as a gradient-based optimization task. In order to accommodate non-differentiability of tree ensembles, we adopt the probabilistic model approximations within the optimization framework. This enables end-to-end unlearning in an effective and efficient manner. Extensive experiments on real-world datasets show that FUTURE yields significant and successful unlearning performance.

==> Attack_Result.tex <==
\begin{table*}[ht!]
.\caption{\label{tab:Result80}
$HR@10\times100$ for different attacks with $80\%$ training data (left) and $30\%$ training data (right) on two datasets.
}

%\vspace{-2mm}
\scalebox{0.75}{
\centering
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$0.34$} & 
\multicolumn{1}{c|}{$0.39$} &
 \multicolumn{1}{c|}{$0.72$} & 
\multicolumn{1}{c|}{$0.82$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.32$} &
\multicolumn{1}{c|}{$0.38$} &
\multicolumn{1}{c|}{$0.79$} & 
\multicolumn{1}{c|}{$0.86$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$\bf{0.37}$} & 
\multicolumn{1}{c|}{$\bf{0.42}$} &
\multicolumn{1}{c|}{$\bf{0.82}$} & 
\multicolumn{1}{c|}{$\bf{0.91}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.11$} &
\multicolumn{1}{c|}{$0.16$} & 
\multicolumn{1}{c|}{$0.26$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.25}$} &
\multicolumn{1}{c|}{$\bf{0.29}$} &
 \multicolumn{1}{c|}{$0.63$} & 
\multicolumn{1}{c|}{$0.71$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$0.28$} &
\multicolumn{1}{c|}{$0.66$} & 
\multicolumn{1}{c|}{$0.73$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$0.24$} & 
\multicolumn{1}{c|}{$\bf{0.29}$} & 
\multicolumn{1}{c|}{$\bf{0.68}$} & 
\multicolumn{1}{c|}{$\bf{0.76}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.10$} &
\multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.14$}
\\

\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$\bf{0.27}$} & 
\multicolumn{1}{c|}{$0.30$} &
 \multicolumn{1}{c|}{$0.63$} & 
\multicolumn{1}{c|}{$0.73$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.25$} &
\multicolumn{1}{c|}{$0.31$} &
\multicolumn{1}{c|}{$0.65$} & 
\multicolumn{1}{c|}{$0.74$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$0.26$} & 
\multicolumn{1}{c|}{$\bf{0.33}$} &
\multicolumn{1}{c|}{$\bf{0.66}$} & 
\multicolumn{1}{c|}{$\bf{0.76}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.08$} &
\multicolumn{1}{c|}{$0.16$} & 
\multicolumn{1}{c|}{$0.21$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.24}$} &
\multicolumn{1}{c|}{$0.25$} &
 \multicolumn{1}{c|}{$0.56$} & 
\multicolumn{1}{c|}{$0.63$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.22$} & 
\multicolumn{1}{c|}{$0.24$} &
\multicolumn{1}{c|}{$0.59$} & 
\multicolumn{1}{c|}{$0.63$} 

\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$\bf{0.26}$} &
\multicolumn{1}{c|}{$\bf{0.61}$} & 
\multicolumn{1}{c|}{$\bf{0.66}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.03$} & 
\multicolumn{1}{c|}{$0.04$} &
\multicolumn{1}{c|}{$0.12$} & 
\multicolumn{1}{c|}{$0.18$}
\\
\cline{2-7}
\hline
\end{tabular}
\quad
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$0.12$} & 
\multicolumn{1}{c|}{$0.14$} &
 \multicolumn{1}{c|}{$0.21$} & 
\multicolumn{1}{c|}{$0.23$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.10$} &
\multicolumn{1}{c|}{$0.14$} &
\multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$0.29$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$\bf{0.13}$} & 
\multicolumn{1}{c|}{$\bf{0.18}$} &
\multicolumn{1}{c|}{$\bf{0.29}$} & 
\multicolumn{1}{c|}{$\bf{0.35}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.02$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.10$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.06}$} &
\multicolumn{1}{c|}{$0.09$} &
 \multicolumn{1}{c|}{$0.17$} & 
\multicolumn{1}{c|}{$0.22$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.04$} & 
\multicolumn{1}{c|}{$0.08$} &
\multicolumn{1}{c|}{$0.17$} & 
\multicolumn{1}{c|}{$0.21$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.06}$} & 
\multicolumn{1}{c|}{$\bf{0.11}$} & 
\multicolumn{1}{c|}{$\bf{0.20}$} & 
\multicolumn{1}{c|}{$\bf{0.26}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.03$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.08$}
\\

\hline

\multicolumn{1}{|l|}{\multirow{8}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$0.05$} &
\multicolumn{1}{c|}{$0.06$} &
 \multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.11$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.05$} &
\multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.12$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.06}$} & 
\multicolumn{1}{c|}{$\bf{0.08}$} & 
\multicolumn{1}{c|}{$\bf{0.12}$} & 
\multicolumn{1}{c|}{$\bf{0.16}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.01$} & 
\multicolumn{1}{c|}{$0.02$} &
\multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.08$}
\\
\cline{2-7}

\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$0.06$} &
\multicolumn{1}{c|}{$0.08$} &
 \multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.15$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.09$} &
\multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.16$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.07}$} & 
\multicolumn{1}{c|}{$\bf{0.10}$} & 
\multicolumn{1}{c|}{$\bf{0.15}$} & 
\multicolumn{1}{c|}{$\bf{0.20}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.02$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.10$}
\\
\cline{2-7}

\hline


\end{tabular}
}
\end{table*}

==> Attack_result30.tex <==
\begin{table*}[ht!]
\caption{\label{tab:Result30}
HR@10$\times$100 for different attacks with $30\%$ training data on two datasets (best performance in bold).
}
\vspace{-2mm}
\scalebox{0.75}{
\centering
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{9}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
\multicolumn{1}{c|}{$0.0012$} & 
\multicolumn{1}{c|}{$0.0014$} &
 \multicolumn{1}{c|}{$0.0021$} & 
\multicolumn{1}{c|}{$0.0023$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
\multicolumn{1}{c|}{$0.0010$} &
\multicolumn{1}{c|}{$0.0014$} &
\multicolumn{1}{c|}{$0.0023$} & 
\multicolumn{1}{c|}{$0.0029$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc H-CARS} &
\multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0018$} &
\multicolumn{1}{c|}{$0.0029$} & 
\multicolumn{1}{c|}{$0.0035$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0002$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0010$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0006$} &
\multicolumn{1}{c|}{$0.0009$} &
 \multicolumn{1}{c|}{$0.0017$} & 
\multicolumn{1}{c|}{$0.0022$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0004$} & 
\multicolumn{1}{c|}{$0.0008$} &
\multicolumn{1}{c|}{$0.0017$} & 
\multicolumn{1}{c|}{$0.0021$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0011$} & 
\multicolumn{1}{c|}{$0.0020$} & 
\multicolumn{1}{c|}{$0.0026$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0003$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0008$}
\\
\cline{2-7}

\hline

\multicolumn{1}{|l|}{\multirow{9}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0005$} &
\multicolumn{1}{c|}{$0.0006$} &
 \multicolumn{1}{c|}{$0.009$} & 
\multicolumn{1}{c|}{$0.0011$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0005$} &
\multicolumn{1}{c|}{$0.009$} & 
\multicolumn{1}{c|}{$0.0012$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0008$} & 
\multicolumn{1}{c|}{$0.0012$} & 
\multicolumn{1}{c|}{$0.0016$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0001$} & 
\multicolumn{1}{c|}{$0.0002$} &
\multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0008$}
\\
\cline{2-7}

\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0006$} &
\multicolumn{1}{c|}{$0.0008$} &
 \multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0015$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0009$} &
\multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0016$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0007$} & 
\multicolumn{1}{c|}{$0.0010$} & 
\multicolumn{1}{c|}{$0.0015$} & 
\multicolumn{1}{c|}{$0.0020$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0002$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0010$}
\\
\cline{2-7}

\hline


\end{tabular}
}
\end{table*}

==> ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}



==> background.tex <==
\section{Background and Preliminaries}
\label{sec:background}
We consider the standard collaborative filtering recommendation task.
Let $\mathcal{U}=\{u_1,\ldots,u_m\}$ be a set of $m$ users, and $\mathcal{I}=\{i_1,\ldots,i_n\}$ be a set of $n$ items.
% User-Item (Rating) Matrix 
We represent the \textit{factual} interactions between users and items with a binary user-item matrix $\mathcal{Y}\in\{0,1\}^{m\times n}$, where $Y_{u,i}=y_{u,i} = 1$ indicates that user $u$ has interacted with item $i$, or $0$ otherwise. Specifically, we denote the interaction history of a user $u$ as $\I_{u}=\{i\in \I~|~y_{u,i} = 1\}$. %$I_{u}=\{i_{u}^{1},i_{u}^{2},\ldots,i_{u}^{l}\}$.

We assume there exists a recommendation model $f$ that can estimate the value $\hat{y}_{u,i}$ for each $u\in \mathcal{U}$ and each $i\in \I$, such that $i\notin \I_u$, as $\hat{y}_{u,i} = f(\h_u, \h_i)$, where $\h_u,\h_i\in \R^d$ are suitable user and item representations, respectively, and $f: \R^d \times \R^d \mapsto [0,1]$ is a function that measures the preference
score for user $u$ on item $i$.\footnote{A similar reasoning would apply if we instead considered explicit ratings, i.e., $f: \R^d \times \R^d \mapsto \R$.}
The predicted score computed with $f$ is, in turn, used to rank items to populate a list $\hat{\I}^k_{u}\subseteq \I\setminus \I_u$ of the top-$k$ recommended items for user $u$, i.e., the list of $k$ unrated items most likely relevant to user $u$ according to $f$.

Thus, given a target item $t$ recommended to a user $u$ by $f$ (i.e., $t\in \hat{\I}^k_{u}$), its counterfactual explanations are the minimal subset of $u$'s historical item interactions $\I_u$ whose removal results in kicking $t$ out of the top-$k$ list of recommendations $\hat{\I}^k_{u}$, namely $\I_{u,t}^{CF} \subset \I_u$.
%\gabri{I'm not sure if we want to keep the requirement on \textit{minimality} in the informal definition above of CFs.}
%given a query on user and target item pair $(u,i_u^{j})$, counterfactual explanations is a set of $u$'s history 
%$I_{(u,i_u^{j})}^{CF}\subset I_{u}$ whose removal results in kicking $i_u^{k}$ out of the top-$k$ list.
 % \gabri{The notation here is a bit confusing and too hard to read! First, the $k$ used as superscript in $i_u^k$ should not be confused with the top-$k$ list, right? If I understand correctly, $i_u^k$ is just a generic item (within the interaction history). Also, the subscript $(u, i_u^k)$ underneath $I^{CF}$ is very annoying.}
 % \ziheng{We also notice that issue but don't know how to simplify it. As we have an attack toward the logic chain, the items in $I_u$ must contain information of both the target user and the target item.  Could you provide us a plausible notation here? I can replace all left by myself.}
 %\gabri{I got that, but, currently, $I_u$ does {\bf not} contain $u$, as it is defined as the set of items which $u$ has interacted with. Also, please be consistent with the abbreviation for counterfactual: you have used both $CF$ and $\mathcal{cf}$ (in the loss below). We could go with something like: "Besides, given a query on user and target item pair $(u,i_{u}^{j})$, the counterfactual explanation is a set of $u$'s history $I_{j}^{CF}\subset I_{u}$ (or, $I_{j}^{\mathcal {cf}}\subset I_{u}$) whose removal results in kicking $i_{u}^{j}$ out of the top-$k$ list." Then, we could specify what you said, namely that we need both $u$ and $I_u$ (in this way, you don't need to have $u$ within $I_u$).} 
 
%\gabri{The attack model is kind of "brutally" introduced (i.e., we start talking about an \textit{attacker} out of the blue, below). We should perhaps think of a way to present this better.}
% I HAVE MOVED THIS PARAGRAPH BELOW TO THE NEXT SECTION (ATTACK MODEL)
%In reality, online service providers restrict one's access to the full user-item interaction data. Hence, our attack model assumes that the factual interaction matrix $\mathcal{Y}$ can only be partially observed. Additionally, recommender systems are generally considered as ``black-boxes'', i.e., the model's internals (i.e., its architecture, parameters, and gradients) are inaccessible to the attacker. 
%Nevertheless, it is common for a recommender system to expose public APIs that can be queried (by the attacker) to generate the top-$k$ list of suggestions for a given user $u$. 
%Furthermore, an explanation API for the recommendation model could also be exploited to produce CFs for any user and target item $(u,t)$.




==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
%In this work, we presented H-CARS, the first poisoning attack to recommender systems that exploits vulnerabilities induced by counterfactual explanations. 

We present FUTURE, a novel model-agnostic, effective and efficient tree-based unlearning methods. It can work with all kinds of tree-based models.

Compared to tree-based unlearning methods, it can be trained end-to-end.

Experiments on two datasets across three types of tree-based models demonstrate the effectiveness of FUTURE.
When there are large number of unlearning requests, FUTURE can maintain 95\% of predictive power, outperforming existing tree-based unlearning methods significantly. 


% We presented a novel approach, H-CARS, that exploits the vulnerabilities induced by counterfactual explanations to launch a poisoning attack on recommender systems. To the best of our knowledge, this is the first such attack proposed in the literature. Our experiments demonstrate that H-CARS is effective, highlighting the importance of considering the security implications of using explainability methods in recommender systems. Future research should explore the potential impact of such attacks on the integrity of the recommender system, as well as develop stronger defenses to mitigate risks in explainable recommender systems.

==> problem.tex <==
%\section{Problem Formulation}
\label{sec:problem}
\section{Attack Model}
\label{sec:problem}
We follow the pipeline of poisoning attack, which aims at promoting target items to as many legitimate users as possible by injecting controlled users with carefully crafted interactions. 
Formally, let $\mathcal{T}\subseteq \I$ denotes the set of target items, $\mathcal{U}$ and $\mathcal{U}'$ denote the set of legitimate users and users controlled by the attacker, respectively. 
%\gabri{We do not use $\mathcal{T}$ anywhere else in the paper, except for here! Do we really need this?}
Accordingly, $\mathcal{Y}$ and $\mathcal{Y}'$ denote the factual and fake interactions. 
It is worth noting that, in practice, online recommender systems restrict one's access to the full user-item interaction data. Hence, our attack model assumes that the factual interaction matrix $\mathcal{Y}$ can only be partially observed. Additionally, recommender systems are generally considered as ``black-boxes'', i.e., the model's internals (i.e., its architecture, parameters, and gradients) are inaccessible to the attacker. 
Nevertheless, it is common for a recommender system to expose a public API that can be queried (by the attacker) to generate the top-$k$ list of suggestions for a given user $u$. 
Furthermore, an explanation API for the recommendation model could also be exploited to produce CFs for any user and target item $(u,t)$.

To quantify the power of the attack, we define its success rate $HR(t)$ -- the hit ratio of item $t\in \mathcal{T}$ -- as the probability that $t$ appears in the top-$k$ list of recommended items for an actual user, i.e., $\mathbb{P}(\{t\in \hat{\I}_u^k~|~u\in \mathcal{U}\})$. 

% $\mathcal{HR}_{t}=\frac{\sum_{u \in \mathcal{U}}\mbox{I}\{t \in I_{u}^{K}\}}{|\mathcal{U}|}$. 
Eventually, the attacker's goal is to craft the fake interactions $\mathcal{Y}'$ for $\mathcal{U}'$, such that the hit ratio of the target items is maximized. Formally, following previous work~\cite{zhang2021data}\cite{huang2021data}, we formulate the bi-level optimization problem as follows:
\begin{equation}
\label{eq:Globalattack}
\begin{aligned}
 \max &
 \sum_{t \in \mathcal{T}}HR(t)\\
%& \textrm{subject to:} \quad |\features| \leq m.
\textrm{subject to: } & \params^{*}=\argmin\limits_{\params}\Big\{\mathcal{L}_{train}(\mathcal{Y},\hat{\mathcal{Y}}_{\params})+\mathcal{L}_{train}(\mathcal{Y}',\hat{\mathcal{Y}}'_{\params})\Big\},
\end{aligned}
\end{equation}
where $\params$ denotes the model parameters, and $\mathcal{L}_{train}$ denotes the training loss of the target recommendation model $f$. $\mathcal{Y}_{\params}$ and $\mathcal{Y}'_{\params}$ are predictions from the model trained on $\mathcal{Y} \cup \mathcal{Y}'$.

==> related.tex <==
\section{Related Work}
\label{sec:related}


==> table.tex <==
\begin{table*}[ht]
\scalebox{0.6}{
\centering
%\begin{tabular}{lll|cc|cc|cc|}
\begin{tabular}{lll|cc|cc|cc|cc|cc|cc|}
%\cline{4-9}
\cline{4-15}
% & & & \multicolumn{2}{c|}{{\bf Top-$10$}} & \multicolumn{2}{c|}{{\bf Top-$15$}} & \multicolumn{2}{c|}{{\bf Top-$20$}}
& & & \multicolumn{4}{c|}{{\bf Top-$10$}} & \multicolumn{4}{c|}{{\bf Top-$15$}} & \multicolumn{4}{c|}{{\bf Top-$20$}}
\\
%\cline{4-9}
\cline{4-15}
% & & & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}} & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}} & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}}
& & & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}} & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}} & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}}
\\
\hline
% \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l|}{\thead{Recommendation\\Model}} & \multicolumn{1}{l|}{\thead{Explanation\\Method}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}}
\multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Explanation\\Method}} & \multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC} &
\multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC} &
\multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC}
\\
\hline
% LastFM
\multicolumn{1}{|l|}{\multirow{12}{*}{\em LastFM}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{${\bf0.62} (\pm 0.05)$} & \multicolumn{1}{c|}{${\bf5.91} (\pm 0.70)$} & \multicolumn{1}{c|}{${\bf0.87} (\pm 0.02)$} &
\multicolumn{1}{c|}{${\bf3.98} (\pm 0.26)$} &
\multicolumn{1}{l|}{${\bf0.56} (\pm 0.05)$} & \multicolumn{1}{c|}{${\bf5.31} (\pm 0.58)$} & \multicolumn{1}{c|}{${\bf0.85} (\pm 0.07)$} &
\multicolumn{1}{c|}{${\bf4.17} (\pm 0.38)$} &
\multicolumn{1}{c|}{${\bf0.55} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.67} (\pm 0.75)$} & \multicolumn{1}{c|}{$\mathbf{0.82} (\pm 0.08)$} &
\multicolumn{1}{c|}{$\mathbf{4.58} (\pm 0.45)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.57 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.30 (\pm 0.40)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.37 (\pm 0.32)$} &
\multicolumn{1}{l|}{$0.54 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 0.35)$} &
\multicolumn{1}{c|}{$0.49 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.11 (\pm 0.70)$} & \multicolumn{1}{c|}{$\mathbf{0.82} (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.66 (\pm 0.45)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.58 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.73 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.55 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.87 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.77 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.31 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.76 (\pm 0.07)$} &
\multicolumn{1}{c|}{$5.79 (\pm 0.32)$}
\\
\cline{3-15}
 \multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.07 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.09 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.02)$} &
\multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} & \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.50 (\pm 0.83)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.90 (\pm 0.35    )$} &
\multicolumn{1}{l|}{$0.55 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.83)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.26 (\pm 0.34)$} &
\multicolumn{1}{c|}{$\mathbf{0.70} (\pm 0.06)$} & \multicolumn{1}{c|}{$\mathbf{6.30} (\pm 0.82)$} & \multicolumn{1}{c|}{$\mathbf{0.86} (\pm 0.09)$} & \multicolumn{1}{c|}{$\mathbf{5.01} (\pm 0.46)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.61 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.70 (\pm 0.82)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.52 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.66 (\pm 0.78)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.68 (\pm 0.35)$} &
\multicolumn{1}{c|}{$0.68 (\pm 0.07)$} &
\multicolumn{1}{c|}{$6.42 (\pm 0.79)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.32 (\pm 0.43)$}
\\
\cline{3-15}
%\multicolumn{1}{|l|}{\textit{LastFM}} &
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{NGCF} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.59 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.37 (\pm 0.42)$} &
\multicolumn{1}{l|}{$0.50 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.79)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.63 (\pm 0.39)$} &
\multicolumn{1}{c|}{$0.58 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.51)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{c|}{${\bf0.47} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.33)$}&
\multicolumn{1}{l|}{$0.12 (\pm 0.02)$} & \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.23 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.09 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & \multicolumn{1}{c|}{$0.10 (\pm 0.03)$} & \multicolumn{1}{c|}{$0.63 (\pm 1.60)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.57 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.33 (\pm 0.32)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.08)$} &
\multicolumn{1}{c|}{$4.77 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.69 (\pm 0.08)$} & \multicolumn{1}{c|}{$8.42 (\pm 0.61)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.08)$} &
\multicolumn{1}{c|}{$7.63 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.06)$} & \multicolumn{1}{c|}{${\bf5.36}(\pm 0.42)$} & \multicolumn{1}{c|}{${\bf0.83} (\pm 0.03)$} & \multicolumn{1}{c|}{${\bf5.23} (\pm 0.42)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{GCMC} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.53 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.66 (\pm 0.35)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.08 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.68 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.49 (\pm 0.59)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.08)$} &
\multicolumn{1}{c|}{$8.19 (\pm 0.98)$} &
\multicolumn{1}{c|}{$0.52 (\pm 0.03)$} &
\multicolumn{1}{c|}{$6.78 (\pm 0.47)$} & 
\multicolumn{1}{c|}{$0.79 (\pm 0.05)$} & 
\multicolumn{1}{c|}{$5.38 (\pm 0.36)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{GCMC} &
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.52 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.37)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.96 (\pm 0.52)$} &
\multicolumn{1}{l|}{$0.67 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.36 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.23 (\pm 0.96)$} &
\multicolumn{1}{c|}{${\bf0.53} (\pm 0.05)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.78 (\pm 0.06)$} & \multicolumn{1}{c|}{$7.45 (\pm 0.53)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.13 (\pm 0.03)$} & \multicolumn{1}{c|}{$8.47 (\pm 0.62)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.18 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.26 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.62 (\pm 1.20)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.02)$} & \multicolumn{1}{c|}{$9.20 (\pm 0.32)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.37)$}
\\
\hline
\hline
% Yelp
\multicolumn{1}{|l|}{\multirow{12}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.56 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.77 (\pm 0.50)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.08)$} &
\multicolumn{1}{c|}{$3.79 (\pm 0.46)$} &
\multicolumn{1}{l|}{$0.67 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.42 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.06)$} &
\multicolumn{1}{c|}{$3.45 (\pm 0.35)$} &
\multicolumn{1}{c|}{$\mathbf{0.58} (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{6.99} (\pm 0.32)$} & \multicolumn{1}{c|}{$\mathbf{0.76} (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{4.28} (\pm 0.38)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
% \multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.56 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.01 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.05$} &
\multicolumn{1}{c|}{$3.92 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.65 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.89 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.21 (\pm 0.36)$} &
\multicolumn{1}{c|}{$0.55 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.32 (\pm 0.33)$} & \multicolumn{1}{c|}{$0.73 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.19 (\pm 0.29)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
% \multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.55 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.96 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.89 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.15 (\pm 0.42)$} &
\multicolumn{1}{l|}{$0.61 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.79 (\pm 0.36)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.52 (\pm 0.73)$} & \multicolumn{1}{c|}{$0.71 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.63 (\pm 0.45)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.16 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.72 (\pm 0.66)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.02)$} &
\multicolumn{1}{c|}{$5.36 (\pm 0.69)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.35 (\pm 0.13)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 1.32)$} &
\multicolumn{1}{c|}{$0.08 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.02 (\pm 0.19)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.01)$} & \multicolumn{1}{c|}{$5.46 (\pm 1.72)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.66 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.37 (\pm 0.51)$} & \multicolumn{1}{c|}{$0.87 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.35 (\pm 1.12)$} &
\multicolumn{1}{l|}{$0.69 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.21 (\pm 0.82)$} & \multicolumn{1}{c|}{$0.91 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.28 (\pm 0.30)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{4.36} (\pm 0.37)$} & 
\multicolumn{1}{c|}{$\mathbf{0.76} (\pm 0.04)$} & 
\multicolumn{1}{c|}{$\mathbf{3.75} (\pm 0.37)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.64(\pm 0.05)$} & \multicolumn{1}{c|}{$8.85 (\pm 0.60)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.06)$} &
\multicolumn{1}{c|}{$7.43 (\pm 0.88)$} &
\multicolumn{1}{l|}{$0.68 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.86 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.76 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.26 (\pm 0.39)$} & \multicolumn{1}{c|}{$0.75 (\pm 0.03)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.38)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.76 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.08)$} &
\multicolumn{1}{c|}{$8.21 (\pm 0.96)$} &
\multicolumn{1}{l|}{$0.59 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.38)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.03)$} &
\multicolumn{1}{c|}{$6.22 (\pm 0.41)$} &
\multicolumn{1}{c|}{${\bf0.55} (\pm 0.04)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.74 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.83 (\pm 0.45)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.18 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.25 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.32 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.01)$} & \multicolumn{1}{c|}{$8.60 (\pm 0.46)$} & \multicolumn{1}{c|}{$0.22 (\pm 0.02)$} &
\multicolumn{1}{c|}{$8.20 (\pm 1.47)$} &
\multicolumn{1}{c|}{$0.06 (\pm 1.00)$} & \multicolumn{1}{c|}{$6.35 (\pm 1.53)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.21 (\pm 1.70)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.63 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.26 (\pm 0.55)$} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.31 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.76 (\pm 0.52)$} &
\multicolumn{1}{c|}{${\bf0.74} (\pm 0.04)$} & \multicolumn{1}{c|}{${\bf4.14} (\pm 0.37)$} & \multicolumn{1}{c|}{$0.70 (\pm 0.06)$} & \multicolumn{1}{c|}{${\bf4.23} (\pm 0.43)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.61 (\pm 0.03)$} & \multicolumn{1}{c|}{$8.09 (\pm 0.58)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.38 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.64 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.82 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.92 (\pm 0.49)$} &
\multicolumn{1}{c|}{$0.72 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.31 (\pm 0.37)$} & \multicolumn{1}{c|}{$0.71 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.36 (\pm 0.32)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{GCMC} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.60 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.16 (\pm 0.75)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.53 (\pm 0.61)$} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.98 (\pm 0.75)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.61)$} &
\multicolumn{1}{c|}{$0.72 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.63 (\pm 0.43)$} & \multicolumn{1}{c|}{${\bf0.71} (\pm 0.06)$} & \multicolumn{1}{c|}{$4.86 (\pm 0.51)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.12 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.53 (\pm 0.66)$} & \multicolumn{1}{c|}{$0.17 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.31 (\pm 1.16)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.42 (\pm 0.57)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.37 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.10 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.43 (\pm 0.23)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.73 (\pm 0.17)$}
\\
\hline
\hline
% Gowalla
\multicolumn{1}{|l|}{\multirow{12}{*}{\em Gowalla}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.72 (\pm 0.07)$} & \multicolumn{1}{c|}{$6.89 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.89 (\pm 0.51)$} &
\multicolumn{1}{l|}{$0.85 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.83 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.95 (\pm 0.09)$} &
\multicolumn{1}{c|}{$6.21 (\pm 0.33)$} &
\multicolumn{1}{c|}{$0.45 (\pm 0.05)$} & \multicolumn{1}{c|}{$\mathbf{5.56} (\pm 0.27)$} & 
\multicolumn{1}{c|}{$\mathbf{0.83} (\pm 0.08)$} & 
\multicolumn{1}{c|}{ $\mathbf{3.75} (\pm 0.37)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.72 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.02 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.96 (\pm 0.47)$} &
\multicolumn{1}{l|}{$0.83 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.18 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.07)$} &
\multicolumn{1}{c|}{$6.38 (\pm 0.28)$} & \multicolumn{1}{c|}{$0.43 (\pm 0.04)$} & \multicolumn{1}{c|}{$5.92 (\pm 0.31)$} &
\multicolumn{1}{c|}{$0.80 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.06 (\pm 0.30)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.72 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.95 (\pm 0.39)$} & \multicolumn{1}{c|}{$0.89(\pm 0.05)$} &
\multicolumn{1}{c|}{$4.79 (\pm 0.56)$} &
\multicolumn{1}{l|}{$0.77 (\pm 0.08)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.12)$} &
\multicolumn{1}{c|}{$6.32 (\pm 0.31)$} &
\multicolumn{1}{c|}{${\bf0.45} (\pm 0.06)$} & \multicolumn{1}{c|}{$5.88 (\pm 0.31)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.06)$} & \multicolumn{1}{c|}{$4.13 (\pm 0.32)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.13 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.15 (\pm 1.32)$} & \multicolumn{1}{c|}{$0.27 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.39 (\pm 1.16)$} &
\multicolumn{1}{l|}{$0.18 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.36 (\pm 0.99)$} & \multicolumn{1}{c|}{$0.27 (\pm 0.09)$} &
\multicolumn{1}{c|}{$7.02 (\pm 1.05)$} &
\multicolumn{1}{c|}{$0.05 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.73 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.01)$} & \multicolumn{1}{c|}{$6.33 (\pm 0.10)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.65 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.43 (\pm 0.72)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.09)$} &
\multicolumn{1}{c|}{$4.89 (\pm 0.51)$} &
\multicolumn{1}{l|}{$0.81 (\pm 0.06)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.97 (\pm 0.04)$} &
\multicolumn{1}{c|}{$6.31 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.50 (\pm 0.09)$} & \multicolumn{1}{c|}{$5.32 (\pm 0.39)$} & \multicolumn{1}{c|}{$\mathbf{0.85} (\pm 0.06)$} & 
\multicolumn{1}{c|}{$\mathbf{4.23} (\pm 0.22)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.65 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.08 (\pm 0.46)$} & \multicolumn{1}{c|}{$0.94 (\pm 0.08)$} &
\multicolumn{1}{c|}{$5.03 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.81 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.56 (\pm 0.27)$} & \multicolumn{1}{c|}{$0.96 (\pm 0.04)$} &
\multicolumn{1}{c|}{$6.39 (\pm 0.31)$} &
\multicolumn{1}{c|}{$0.49 (\pm 0.07)$} & \multicolumn{1}{c|}{$5.39 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.49 (\pm 0.22)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.65 (\pm 0.07)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.58)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.08)$} &
\multicolumn{1}{c|}{$6.22 (\pm 0.52)$} &
\multicolumn{1}{l|}{$0.79 (\pm 0.09)$} & \multicolumn{1}{c|}{$7,65 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.96 (\pm 0.08)$} &
\multicolumn{1}{c|}{$6.42 (\pm 0.34)$} &
\multicolumn{1}{c|}{${\bf0.51} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.27} (\pm 0.52)$} & \multicolumn{1}{c|}{${\bf0.85} (\pm 0.04)$} & \multicolumn{1}{c|}{$4.39 (\pm 0.26)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.15 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.60 (\pm 0.53)$} & \multicolumn{1}{c|}{$0.22 (\pm 0.03)$} &
\multicolumn{1}{c|}{$8.20 (\pm 1.47)$} &
\multicolumn{1}{l|}{$0.13 (\pm 0.05)$} & \multicolumn{1}{c|}{$8.37 (\pm 0.49)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.15 (\pm 0.77)$} &
\multicolumn{1}{c|}{$0.09 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.32 (\pm 0.45)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.57 (\pm 0.16)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} &
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.58 (\pm 0.05)$} & \multicolumn{1}{c|}{$8.43 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.87 (\pm 0.08)$} &
\multicolumn{1}{c|}{$7.68 (\pm 0.97)$} &
\multicolumn{1}{l|}{$0.60 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.75 (\pm 0.53)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.09)$} &
\multicolumn{1}{c|}{$7.75 (\pm 1.05)$} &
\multicolumn{1}{c|}{$0.46 (\pm 0.09)$} & \multicolumn{1}{c|}{$5.85 (\pm 0.33)$} & \multicolumn{1}{c|}{${\bf0.82} (\pm 0.04)$} & \multicolumn{1}{c|}{${\bf4.32} (\pm 0.29)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.59 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.68 (\pm 0.45)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$8.16 (\pm 0.86)$} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.56 (\pm 0.48)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.15 (\pm 0.83)$} &
\multicolumn{1}{c|}{$0.45 (\pm 0.07)$} & \multicolumn{1}{c|}{$5.93 (\pm 0.31)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.27 (\pm 0.26)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.76 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.21 (\pm 0.96)$} &
\multicolumn{1}{l|}{$0.61 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.83 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.32 (\pm 0.88)$} &
\multicolumn{1}{c|}{${\bf0.47} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.33)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.18 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.25 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.32 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.20 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.38 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.28 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.28 (\pm 1.20)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.01)$} & \multicolumn{1}{c|}{$8.23 (\pm 0.57)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.03)$} & \multicolumn{1}{c|}{$5.00 (\pm 0.96)$}
\\
\hline
\end{tabular}
}
\caption{\label{tab:all-results}
PS($\uparrow$), PN($\uparrow$), and EC($\downarrow$) of factual and counterfactual explanations generated by \textsc{\textbf{GREASE}}, \textsc{\textbf{PGExplainer}}, \textsc{\textbf{PersonalRank}}, and \textsc{\textbf{Random}} for top-$10$, top-$15$, and top-$20$ recommended items according to LightGCN, NGCF, and GCMC GNN-based recommender systems trained on \textit{LastFM}, \textit{Yelp}, and \textit{Gowalla} datasets.}
%\vspace{-3mm}
\end{table*}
